The Effect of Distortions on the Prediction of Visual Attention

Existing saliency models have been designed and evaluated for predicting the saliency in distortion-free images. However, in practice, the image quality is affected by a host of factors at several stages of the image processing pipeline such as acquisition, compression and transmission. Several studies have explored the effect of distortion on human visual attention; however, none of them have considered the performance of visual saliency models in the presence of distortion. Furthermore, given that one potential application of visual saliency prediction is to aid pooling of objective visual quality metrics, it is important to compare the performance of existing saliency models on distorted images. In this paper, we evaluate several state-of-the-art visual attention models over different databases consisting of distorted images with various types of distortions such as blur, noise and compression with varying levels of distortion severity. This paper also introduces new improved performance evaluation metrics that are shown to overcome shortcomings in existing performance metrics. We find that the performance of most models improves with moderate and high levels of distortions as compared to the near distortion-free case. In addition, model performance is also found to decrease with an increase in image complexity.

==> README <==
January 10, 2007

Please note that you may choose to use either double column or single column
formatting. You may wish to use single column formatting when submitting your
paper for review, as it leaves more space for reviewer remarks. The double column format 
is ideal when submitting your final publication materials. The IEEE CS formats articles
in two columns, with 9.5pt Palatino font, and a page size of 7.875 X 10.75. 

June 6, 2006

Added an option to switch between peer review and final submission formats 
into bare_jrnl.tex. 


August 13, 2002

This IEEEtran.cls is the official LaTeX class for authors of the
Institute of Electrical and Electronics Engineers (IEEE) transactions
journals and conferences. In addition to being carried on IEEE's site,
IEEEtran.cls may be found at:

http://www.ctan.org/tex-archive/macros/latex/contrib/supported/IEEEtran/

The CTAN site may have additional files related to non-IEEE uses of this
tool.

As of version 1.6, IEEEtran.cls now provides support for conferences and
A4 paper. Users of previous versions should no longer manually alter margins,
paper sizes, page styles, etc. Also, please note that \author is used
slightly differently from that of V1.5, especially for conferences.
\pubid (if used) must now be placed before \maketitle. \cite is now robust
and can be used within captions without a proceeding \protect.

As with previous versions, The itemize, enumerate, and description lists as
well as \appendix(ces) have enhanced controls and work slightly differently
than is done in traditional LaTeX.

Extensive formal documentation is now available. Enjoy! ;) The appendices
of the user manual contain important information on avoiding commonly
made mistakes, compatibility issues and installation instructions.


Best wishes for all your publication endeavors,

Michael Shell
mshell@ece.gatech.edu



********************* Files **********************

README               - This file.

IEEEtran.cls         - The LaTeX class file.

IEEEtran_HOWTO.pdf   - The user manual.

bare_jrnl.tex        - A "bare bones" starter file for journal papers.




**********************************************************************
 Legal Notice:
 This code and advice is offered as-is without any warranty either
 expressed or implied; without even the implied warranty of
 MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE!
 User assumes all risk.
 In no event shall IEEE or any contributor to this code
 be liable for any damages or losses, including, but not limited to,
 incidental, consequential, or any other damages, resulting from the
 use or misuse of any information contained here.
 
 All statements made here are the opinions of their respective
 authors and are not necessarily endorsed by the IEEE.

 This code/text is distributed under the Perl Artistic License 
 ( http://language.perl.com/misc/Artistic.html ) 
 and may be freely used, distributed and modified.
 Retain all contribution notices and credits.
**********************************************************************



